PThammer: Cross-User-Kernel-Boundary Rowhammer through Implicit Accesses

Rowhammer is a hardware vulnerability in DRAM memory, where repeated access to memory can induce bit flips in neighboring memory locations. Being a hardware vulnerability, rowhammer bypasses all of the system memory protection, allowing adversaries to compromise the integrity and confidentiality of data. Rowhammer attacks have shown to enable privilege escalation, sandbox escape, and cryptographic key disclosures. Recently, several proposals suggest exploiting the spatial proximity between the accessed memory location and the location of the bit flip for a defense against rowhammer. These all aim to deny the attacker's permission to access memory locations near sensitive data. In this paper, we question the core assumption underlying these defenses. We present PThammer, a confused-deputy attack that causes accesses to memory locations that the attacker is not allowed to access. Specifically, PThammer exploits the address translation process of modern processors, inducing the processor to generate frequent accesses to protected memory locations. We implement PThammer, demonstrating that it is a viable attack, resulting in a system compromise (e.g., kernel privilege escalation). We further evaluate the effectiveness of proposed software-only defenses showing that PThammer can overcome those.

==> Makefile <==
# Generic paper Makefile
#
# For usage hints, "make help"
#
#  To create a LaTeX diff against the hg "tip" revision, use the target
#  "diff" (or "viewdiff").
#  To use a revision other than "tip", speciff DIFF=x on the 
#  make command line to choose the revision x.
#

# Verbosity
ifeq (${V},1)
Q:=
else
Q:=@
endif

.PHONY: all

BIBDIR     ?= /home/disy/lib/BibTeX:../../../bibtex:../bibtex
LaTeXEnv   = TEXINPUTS=".:/home/disy/lib/TeX:/home/disy/lib/ps:${TEXINPUTS}:"
BibTexEnv  = BIBINPUTS=".:${BIBDIR}:${BIBINPUTS}:"
BibFiles   = defs-abbrev,extra,combined,systems,fm,other

LaTeX      = ${LaTeXEnv} pdflatex -interaction=nonstopmode
LaTeXdiff  = ./tools/latexdiff
BibTeX     = ${BibTexEnv} bibtex
Fig2Eps    = fig2dev -L eps
Dia2Eps    = dia -t eps -e
AS         = $(shell which as)
CC         = $(shell which gcc)
GnuPlot	   = gnuplot
Inkscape   = $(shell which inkscape)
Eps2Pdf	   = epstopdf --outfile
PdfView	   = xpdf
Pdf2Ps	   = pdf2ps
RmCR       = tr -d '\r'
sed        = $(shell which sed)
#PdfView    = open -a preview
#PdfView    = acroread 
Lpr 	   = lpr
mv	   = mv
awk	   = awk
R	   = R

# Use either "report" or "paper", depending on the template.
# To add a further target, simply append the basename of the .tex file here
Targets    = main
SRCS = bkgd.tex  conclusion.tex  discuss.tex  eva.tex	intro.tex  main.tex  overview.tex  revision.tex 


# CONFIGURATION OPTIONS
# =====================

# For ACM SIG camera ready submission. This will only work if Target
# is a single identifier. You should then be able to use the "camera" target,
# after setting CamRoot appropriately. Answer "no" for re-making references.bib
# Set CamRoot as the filename root per publisher's instructions.
# Should be <paperno>-<lastname-of-first-author>
CamRoot    = <paperno>-<last>
CamDir	   = cameraready

# Any other stuff that may be needed

# END CONFIGURATION OPTIONS
# =========================

Optional = $(addsuffix -diff, $(Targets))
All = $(Targets) $(Optional)
Diffopts= #--type=BWUNDERLINE #-c .latexdiffconfig --append-safecmd="Comment"

Gnuplot_Sources = $(wildcard figures/*.gnuplot)
Figures = $(Gnuplot_Sources:.gnuplot=.pdf)



Pdf = $(addsuffix .pdf, $(Targets))
Tex = $(addsuffix .tex, $(Targets))
Diff_Pdf = $(addsuffix .pdf, $(Optional))

.PHONY: FORCE

all: pdf
diff: diff_pdf
FORCE: pdf
ps: $(Ps)
pdf: $(Figures) Makefile $(Pdf)
diff_pdf: $(Figures) Makefile $(Diff_Pdf)

%.pdf: %.perf tools/bargraph.pl
	@echo $< '->' $@
	${Q} ${BarGraph} -pdf $< > $@

%.pdf: %.eps
	@echo $< '->' $@
	${Q} ${Eps2Pdf} $@ $<

%.pdf: %.ps
	@echo $< '->' $@
	${Q} ${Eps2Pdf} $@ $<

%.eps: %.svg
	@echo $< '->' $@
	${Q} $(if ${Inkscape},,echo "You need inkscape installed to build $@" >&2; exit 1)
	${Q} ${Inkscape} -f $< -D -z -E $@ > /dev/null 2>&1

%.pdf: %.svg
	@echo $< '->' $@
	${Q} $(if ${Inkscape},,echo "You need inkscape installed to build $@" >&2; exit 1)
	${Q} ${Inkscape} -f $< -D -z -A $@ > /dev/null 2>&1

# This target allows you to add figures which have the extension .c_pp that
# correspond to .c sources. Your .c sources can use the lines '/*<*/' and
# '/*>*/' to surround parts of the source you don't want shown in your PDF.
# This allows you to write a .c file that can be compile-checked here and then
# remove extraneous lines for display.
%.c_pp: %.c
	@echo $< '->' $@
	${Q}$(if ${CC},${CC} -c "$<" -o /dev/null,)
	${Q}${sed} -e '/\/\*<\*\//,/\/\*>\*\//d' "$<" >"$@"

%.s_pp: %.s
	@echo $< '->' $@
	${Q}$(if ${AS},${AS} -c "$<" -o /dev/null,)
	${Q}${sed} -e '/\/\*<\*\//,/\/\*>\*\//d' "$<" >"$@"

%.eps: %.dia
	@echo $< '->' $@
	${Q} ${Dia2Eps} $@ $<

%.eps: %.fig
	@echo $< '->' $@
	${Q} ${Fig2Eps} $< $@

%.eps: %.gnuplot
	@echo $< '->' $@
	${Q} ${GnuPlot} $<

%.eps: %.r
	@echo $< '->' $@
	${Q} ${R} --vanilla < $<

%.pdf: %.pdf-shipped
	cp $< $@

view: pdf
	${Q}for i in $(Pdf); do \
		$(PdfView) $$i & \
	done

viewdiff: diff
	${Q}for i in $(Diff_Pdf); do \
		$(PdfView) $$i & \
	done

print: pdf
	${Q}for i in $(Pdf); do \
		$(Lpr) $$i \
	done

clean:
	rm -f *.aux *.toc *.bbl *.blg *.dvi *.log *.pstex* *.eps *.cb *.brf \
		*.idx *.out *.ps *-diff.* *.mps .log *.diff main.pdf

help:
	@echo "Main targets: all diff camera view viewdiff print clean realclean tar"
	@echo "'make diff' will show changes to head revision"
	@echo "'make DIFF=<rev> diff' will show changes to revision <rev>"
	@echo "Avoid TeX \def with arguments, this breaks latexdiff (use \newcommand)"


##############################################################################

DIFF ?= tip

%-diff.dvi: %-diff.tex

%-diff.tex: %.tex FORCE
	@echo "====> Retrieving revision $(DIFF) of $<"
	hg cat -r $(DIFF) $<  > $(@:-diff.tex=-$(DIFF)-diff.tex)
	@echo "====> Creating diff of revision $(DIFF) of $<"
	$(LaTeXdiff) $(Diffopts) $(@:-diff.tex=-$(DIFF)-diff.tex) $< | \
	${RmCR} > $@

.PHONY: FORCE
FORCE:

# don't delete %.aux intermediates
.SECONDARY:

##############################################################################

Rerun = '(There were undefined (references|citations)|Rerun to get (cross-references|the bars) right)'
Rerun_Bib = 'No file.*\.bbl|Citation.*undefined'
Undefined = '((Reference|Citation).*undefined)|(Label.*multiply defined)'
Error = '^! '


%.pdf: %.tex  $(Figures) Makefile ${SRCS}
	${Q}if ! test -e $*.bbl || test $*.bib -nt $*.bbl; then rm -f $*.bbl; fi
	@echo "====> LaTeX first pass: $(<)"
	${Q}$(LaTeX) $< >.log || if egrep -q $(Error) $*.log ; then cat .log; rm $@; false ; fi
	${Q}if egrep -q $(Rerun_Bib) $*.log ; then echo "====> BibTex" && ( $(BibTeX) $* > .log || ( cat .log ; false ) ) && echo "====> LaTeX BibTeX pass" && $(LaTeX) >.log $< || if egrep -q $(Error) $*.log ; then cat .log; rm $@; false ; fi ; fi
	${Q}if egrep -q $(Rerun) $*.log ; then echo "====> LaTeX rerun" && $(LaTeX) >.log $<; fi
	${Q}if egrep -q $(Rerun) $*.log ; then echo "====> LaTeX rerun" && $(LaTeX) >.log $<; fi
	${Q}if egrep -q $(Rerun) $*.log ; then echo "====> LaTeX rerun" && $(LaTeX) >.log $<; fi
	${Q}if [ -a .NeedGS ]; then gs -dSAFER -dBATCH -dNOPAUSE  -sDEVICE=pdfwrite -sOutputFile=tmp.pdf $@; mv tmp.pdf $@; fi
	@echo "====> Undefined references and citations in $(<):"
	@egrep -i $(Undefined) $*.log || echo "None."
	@echo "====> Dimensions:"
	@grep "dimension:" $*.log || echo "None."

##############################################################################
# Generate a list of FIXMEs 
fixmes: 
	${Q}for i in $(Tex); do \
		echo "FIXMEs in $$i:"; \
		nl -b a $$i | grep "FIXME{" | nl -b a; \
		echo -n "Total FIXMES: " && grep "FIXME{" $$i | wc -l; \
		echo; \
	done

usb.pdf: dtrt.sty

